Off Environment Evaluation Using Convex Risk Minimization

Applying reinforcement learning (RL) methods on robots typically involves training a policy in simulation and deploying it on a robot in the real world. Because of the model mismatch between the real world and the simulator, RL agents deployed in this manner tend to perform suboptimally. To tackle this problem, researchers have developed robust policy learning algorithms that rely on synthetic noise disturbances. However, such methods do not guarantee performance in the target environment. We propose a convex risk minimization algorithm to estimate the model mismatch between the simulator and the target domain using trajectory data from both environments. We show that this estimator can be used along with the simulator to evaluate performance of an RL agents in the target domain, effectively bridging the gap between these two environments. We also show that the convergence rate of our estimator to be of the order of ${n^{-1/4}}$, where $n$ is the number of training samples. In simulation, we demonstrate how our method effectively approximates and evaluates performance on Gridworld, Cartpole, and Reacher environments on a range of policies. We also show that the our method is able to estimate performance of a 7 DOF robotic arm using the simulator and remotely collected data from the robot in the real world.

==> Cartpole/cartpole_eval_trained5.0.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0,0.266666666666667,0.105882352941176}
\definecolor{color1}{rgb}{0.0313725490196078,0.250980392156863,0.505882352941176}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.03,0.03)}, anchor=south west, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Epsilon $(\varepsilon)$},
xmajorgrids,
xmin=-0.05, xmax=1.05,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Average Returns},
ymajorgrids,
ymin=0.112208367928119, ymax=0.662466286424228,
ytick style={color=black},
ytick={0.1,0.2,0.3,0.4,0.5,0.6,0.7},
yticklabels={0.1,0.2,0.3,0.4,0.5,0.6,0.7}
]
\path [draw=black, fill=black, opacity=0.1]
(axis cs:0,0.629501423509269)
--(axis cs:0,0.618683913963555)
--(axis cs:0.2,0.590147229075663)
--(axis cs:0.4,0.494982777988883)
--(axis cs:0.6,0.368895638273284)
--(axis cs:0.8,0.253353505954434)
--(axis cs:1,0.220809055937139)
--(axis cs:1,0.243141745341365)
--(axis cs:1,0.243141745341365)
--(axis cs:0.8,0.280387861894022)
--(axis cs:0.6,0.4006291650932)
--(axis cs:0.4,0.527196012927655)
--(axis cs:0.2,0.609014500446594)
--(axis cs:0,0.629501423509269)
--cycle;

\path [draw=color0, fill=color0, opacity=0.1]
(axis cs:0,0.415876758020757)
--(axis cs:0,0.382934630933517)
--(axis cs:0.2,0.300637785000307)
--(axis cs:0.4,0.202456736799108)
--(axis cs:0.6,0.190215462577879)
--(axis cs:0.8,0.138934727463838)
--(axis cs:1,0.137220091496124)
--(axis cs:1,0.150249728085991)
--(axis cs:1,0.150249728085991)
--(axis cs:0.8,0.155890177954385)
--(axis cs:0.6,0.218845411462586)
--(axis cs:0.4,0.232026334763921)
--(axis cs:0.2,0.32962114906531)
--(axis cs:0,0.415876758020757)
--cycle;

\path [draw=red!49.8039215686275!black, fill=red!49.8039215686275!black, opacity=0.1]
(axis cs:0,0.633967658726771)
--(axis cs:0,0.633967658726771)
--(axis cs:0.2,0.633967658726771)
--(axis cs:0.4,0.633967658726771)
--(axis cs:0.6,0.633967658726771)
--(axis cs:0.8,0.633967658726771)
--(axis cs:1,0.633967658726771)
--(axis cs:1,0.633967658726771)
--(axis cs:1,0.633967658726771)
--(axis cs:0.8,0.633967658726771)
--(axis cs:0.6,0.633967658726771)
--(axis cs:0.4,0.633967658726771)
--(axis cs:0.2,0.633967658726771)
--(axis cs:0,0.633967658726771)
--cycle;

\addplot [ultra thick, black, dashed]
table {%
0 0.624092668736412
0.2 0.599580864761128
0.4 0.511089395458269
0.6 0.384762401683242
0.8 0.266870683924228
1 0.231975400639252
};
\addlegendentry{True Value}
\addplot [ultra thick, color0]
table {%
0 0.399405694477137
0.2 0.315129467032809
0.4 0.217241535781514
0.6 0.204530437020233
0.8 0.147412452709112
1 0.143734909791057
};
\addlegendentry{OEE (ours)}
\addplot [ultra thick, red!49.8039215686275!black]
table {%
0 0.633967658726771
0.2 0.633967658726771
0.4 0.633967658726771
0.6 0.633967658726771
0.8 0.633967658726771
1 0.633967658726771
};
\addlegendentry{MLE}
\addplot [ultra thick, color1]
table {%
0.2 0.265727233222893
0.4 0.633723168651689
0.6 0.637222450529576
0.8 0.637253008577106
1 0.637454562856223
};
\addlegendentry{IS}
\end{axis}

\end{tikzpicture}


==> DartEnv/dart_evaluation_2142.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0,0.266666666666667,0.105882352941176}
\definecolor{color3}{rgb}{0.2549, 0.6823, 0.4627}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Theta},
xmajorgrids,
xmin=-1.15191730631626, xmax=1.15191730631626,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Average returns},
ymajorgrids,
ymin=-99.2405501408194, ymax=3.15670128247421,
ytick style={color=black}
]
\path [draw=black, fill=black, opacity=0.1]
(axis cs:-1.0471975511966,-28.6907700848396)
--(axis cs:-1.0471975511966,-38.894051498729)
--(axis cs:-0.936966230018008,-40.6094873077964)
--(axis cs:-0.826734908839419,-42.2803661393423)
--(axis cs:-0.71650358766083,-41.9556818072214)
--(axis cs:-0.606272266482241,-40.7584584797594)
--(axis cs:-0.496040945303652,-32.9862328408154)
--(axis cs:-0.385809624125062,-26.290572175141)
--(axis cs:-0.275578302946473,-16.0178815494954)
--(axis cs:-0.165346981767884,-14.1109662609134)
--(axis cs:-0.0551156605892946,-24.1754331748587)
--(axis cs:0.0551156605892946,-36.2042117842115)
--(axis cs:0.165346981767884,-46.9381786251432)
--(axis cs:0.275578302946473,-52.6302902573097)
--(axis cs:0.385809624125062,-62.1253682244447)
--(axis cs:0.496040945303651,-68.8227206990797)
--(axis cs:0.606272266482241,-69.8630559750889)
--(axis cs:0.71650358766083,-71.5815350825162)
--(axis cs:0.826734908839419,-70.9209370138817)
--(axis cs:0.936966230018008,-65.0221731310904)
--(axis cs:1.0471975511966,-57.7488926280139)
--(axis cs:1.0471975511966,-47.3888800313253)
--(axis cs:1.0471975511966,-47.3888800313253)
--(axis cs:0.936966230018008,-54.3625907314019)
--(axis cs:0.826734908839419,-57.5177886976029)
--(axis cs:0.71650358766083,-56.4654569871052)
--(axis cs:0.606272266482241,-55.0185519416719)
--(axis cs:0.496040945303651,-50.3715634326795)
--(axis cs:0.385809624125062,-45.3316968819678)
--(axis cs:0.275578302946473,-35.2220006412171)
--(axis cs:0.165346981767884,-25.8839343032337)
--(axis cs:0.0551156605892946,-16.1639044325849)
--(axis cs:-0.0551156605892946,-5.09114163656291)
--(axis cs:-0.165346981767884,-1.49771923676641)
--(axis cs:-0.275578302946473,-2.41162933206079)
--(axis cs:-0.385809624125062,-6.89134854209811)
--(axis cs:-0.496040945303652,-15.9377139287872)
--(axis cs:-0.606272266482241,-20.2020526625158)
--(axis cs:-0.71650358766083,-26.7905742301993)
--(axis cs:-0.826734908839419,-29.3794622718417)
--(axis cs:-0.936966230018008,-28.6921057352699)
--(axis cs:-1.0471975511966,-28.6907700848396)
--cycle;

\path [draw=color0, fill=color0, opacity=0.1]
(axis cs:-1.0471975511966,-12.7921121018969)
--(axis cs:-1.0471975511966,-21.221849761686)
--(axis cs:-0.936966230018008,-36.4662398863668)
--(axis cs:-0.826734908839419,-38.2679169338815)
--(axis cs:-0.71650358766083,-40.7354753333094)
--(axis cs:-0.606272266482241,-33.0147075958838)
--(axis cs:-0.496040945303652,-23.250325705658)
--(axis cs:-0.385809624125062,-18.1564055985287)
--(axis cs:-0.275578302946473,-11.7052420788526)
--(axis cs:-0.165346981767884,-10.12319255789)
--(axis cs:-0.0551156605892946,-17.154946281228)
--(axis cs:0.0551156605892946,-26.5374836010709)
--(axis cs:0.165346981767884,-38.1491706708179)
--(axis cs:0.275578302946473,-48.8487497648236)
--(axis cs:0.385809624125062,-59.2470678770581)
--(axis cs:0.496040945303651,-67.0138082387168)
--(axis cs:0.606272266482241,-68.4036418201015)
--(axis cs:0.71650358766083,-64.0562571889732)
--(axis cs:0.826734908839419,-68.6885810177613)
--(axis cs:0.936966230018008,-75.3665416307967)
--(axis cs:1.0471975511966,-84.0393153921289)
--(axis cs:1.0471975511966,-50.8669528251571)
--(axis cs:1.0471975511966,-50.8669528251571)
--(axis cs:0.936966230018008,-47.0738271112957)
--(axis cs:0.826734908839419,-41.5069850622738)
--(axis cs:0.71650358766083,-43.8332865808095)
--(axis cs:0.606272266482241,-47.6412847321829)
--(axis cs:0.496040945303651,-40.3325053729228)
--(axis cs:0.385809624125062,-40.8295816019166)
--(axis cs:0.275578302946473,-34.3824432608369)
--(axis cs:0.165346981767884,-29.4686350850735)
--(axis cs:0.0551156605892946,-20.5566793306242)
--(axis cs:-0.0551156605892946,-13.6650052004572)
--(axis cs:-0.165346981767884,-8.74234868075722)
--(axis cs:-0.275578302946473,-8.54894647719296)
--(axis cs:-0.385809624125062,-11.0135496577129)
--(axis cs:-0.496040945303652,-16.7539531941137)
--(axis cs:-0.606272266482241,-23.2246788969515)
--(axis cs:-0.71650358766083,-28.7856630996153)
--(axis cs:-0.826734908839419,-29.8745702461062)
--(axis cs:-0.936966230018008,-26.1288475189328)
--(axis cs:-1.0471975511966,-12.7921121018969)
--cycle;

\path [draw=red!49.8039215686275!black, fill=red!49.8039215686275!black, opacity=0.1]
(axis cs:-1.0471975511966,-13.4018064712788)
--(axis cs:-1.0471975511966,-34.3253641126437)
--(axis cs:-0.936966230018008,-36.861056718685)
--(axis cs:-0.826734908839419,-34.7607830501671)
--(axis cs:-0.71650358766083,-35.3244244478396)
--(axis cs:-0.606272266482241,-30.0387521125554)
--(axis cs:-0.496040945303652,-27.2836855049268)
--(axis cs:-0.385809624125062,-29.0567216256592)
--(axis cs:-0.275578302946473,-28.0929747620641)
--(axis cs:-0.165346981767884,-43.4530062402024)
--(axis cs:-0.0551156605892946,-52.7408558185807)
--(axis cs:0.0551156605892946,-63.9708220156813)
--(axis cs:0.165346981767884,-73.1516033990932)
--(axis cs:0.275578302946473,-83.9571460229945)
--(axis cs:0.385809624125062,-89.9286428008505)
--(axis cs:0.496040945303651,-93.8174900355995)
--(axis cs:0.606272266482241,-94.5861296215787)
--(axis cs:0.71650358766083,-94.0141513356309)
--(axis cs:0.826734908839419,-89.4805760294973)
--(axis cs:0.936966230018008,-82.3551091598751)
--(axis cs:1.0471975511966,-72.7277969078669)
--(axis cs:1.0471975511966,-52.0180130273239)
--(axis cs:1.0471975511966,-52.0180130273239)
--(axis cs:0.936966230018008,-59.3651517909715)
--(axis cs:0.826734908839419,-65.9260446867152)
--(axis cs:0.71650358766083,-65.9233281322332)
--(axis cs:0.606272266482241,-61.6436362853984)
--(axis cs:0.496040945303651,-59.4910602095377)
--(axis cs:0.385809624125062,-54.5109374752628)
--(axis cs:0.275578302946473,-47.8770495800246)
--(axis cs:0.165346981767884,-36.480309911283)
--(axis cs:0.0551156605892946,-24.1258240012864)
--(axis cs:-0.0551156605892946,-18.168358023642)
--(axis cs:-0.165346981767884,-9.87169817988281)
--(axis cs:-0.275578302946473,-3.84151947626349)
--(axis cs:-0.385809624125062,-6.53721287042797)
--(axis cs:-0.496040945303652,-3.44238552139544)
--(axis cs:-0.606272266482241,-4.1687477308499)
--(axis cs:-0.71650358766083,-8.50305637044154)
--(axis cs:-0.826734908839419,-12.3500495106441)
--(axis cs:-0.936966230018008,-13.9142315116628)
--(axis cs:-1.0471975511966,-13.4018064712788)
--cycle;

\addplot [ultra thick, black, dashed]
table {%
-1.0471975511966 -33.7924107917843
-0.936966230018008 -34.6507965215332
-0.826734908839419 -35.829914205592
-0.71650358766083 -34.3731280187103
-0.606272266482241 -30.4802555711376
-0.496040945303652 -24.4619733848013
-0.385809624125062 -16.5909603586196
-0.275578302946473 -9.21475544077812
-0.165346981767884 -7.80434274883992
-0.0551156605892946 -14.6332874057108
0.0551156605892946 -26.1840581083982
0.165346981767884 -36.4110564641884
0.275578302946473 -43.9261454492634
0.385809624125062 -53.7285325532063
0.496040945303651 -59.5971420658796
0.606272266482241 -62.4408039583804
0.71650358766083 -64.0234960348107
0.826734908839419 -64.2193628557423
0.936966230018008 -59.6923819312461
1.0471975511966 -52.5688863296696
};
\addlegendentry{True Value}
\addplot [ultra  thick, color0, mark=*, mark size=2.0, mark options={solid,fill=color3}]
table {%
-1.0471975511966 -17.0069809317914
-0.936966230018008 -31.2975437026498
-0.826734908839419 -34.0712435899939
-0.71650358766083 -34.7605692164623
-0.606272266482241 -28.1196932464176
-0.496040945303652 -20.0021394498858
-0.385809624125062 -14.5849776281208
-0.275578302946473 -10.1270942780228
-0.165346981767884 -9.43277061932359
-0.0551156605892946 -15.4099757408426
0.0551156605892946 -23.5470814658476
0.165346981767884 -33.8089028779457
0.275578302946473 -41.6155965128303
0.385809624125062 -50.0383247394874
0.496040945303651 -53.6731568058198
0.606272266482241 -58.0224632761422
0.71650358766083 -53.9447718848913
0.826734908839419 -55.0977830400176
0.936966230018008 -61.2201843710462
1.0471975511966 -67.453134108643
};
\addlegendentry{OEE (ours)}
\addplot [ultra thick, red!49.8039215686275!black]
table {%
-1.0471975511966 -23.8635852919613
-0.936966230018008 -25.3876441151739
-0.826734908839419 -23.5554162804056
-0.71650358766083 -21.9137404091406
-0.606272266482241 -17.1037499217026
-0.496040945303652 -15.3630355131611
-0.385809624125062 -17.7969672480436
-0.275578302946473 -15.9672471191638
-0.165346981767884 -26.6623522100426
-0.0551156605892946 -35.4546069211113
0.0551156605892946 -44.0483230084838
0.165346981767884 -54.8159566551881
0.275578302946473 -65.9170978015095
0.385809624125062 -72.2197901380566
0.496040945303651 -76.6542751225686
0.606272266482241 -78.1148829534886
0.71650358766083 -79.9687397339321
0.826734908839419 -77.7033103581062
0.936966230018008 -70.8601304754233
1.0471975511966 -62.3729049675954
};
\addlegendentry{Simulated}
\end{axis}

\end{tikzpicture}


==> DartEnv/dart_evaluation_3142.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0,0.266666666666667,0.105882352941176}
\definecolor{color3}{rgb}{0.2549, 0.6823, 0.4627}
\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Theta},
xmajorgrids,
xmin=-1.15191730631626, xmax=1.15191730631626,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Average returns},
ymajorgrids,
ymin=-103.522494691815, ymax=2.77641409244283,
ytick style={color=black}
]
\path [draw=black, fill=black, opacity=0.1]
(axis cs:-1.0471975511966,-22.7519982348471)
--(axis cs:-1.0471975511966,-32.7813086099829)
--(axis cs:-0.936966230018008,-36.0039447665112)
--(axis cs:-0.826734908839419,-36.0247104141883)
--(axis cs:-0.71650358766083,-33.9690047650466)
--(axis cs:-0.606272266482241,-30.7489280419564)
--(axis cs:-0.496040945303652,-24.9438333173479)
--(axis cs:-0.385809624125062,-15.3112376009949)
--(axis cs:-0.275578302946473,-13.8593140919826)
--(axis cs:-0.165346981767884,-23.2028381933359)
--(axis cs:-0.0551156605892946,-34.298509482855)
--(axis cs:0.0551156605892946,-45.0471220449742)
--(axis cs:0.165346981767884,-54.6122166685312)
--(axis cs:0.275578302946473,-64.706506687987)
--(axis cs:0.385809624125062,-71.3922932983564)
--(axis cs:0.496040945303651,-76.4591944123726)
--(axis cs:0.606272266482241,-80.3958886003913)
--(axis cs:0.71650358766083,-80.1741208725266)
--(axis cs:0.826734908839419,-75.7417500251848)
--(axis cs:0.936966230018008,-71.8371682272835)
--(axis cs:1.0471975511966,-63.9331416010243)
--(axis cs:1.0471975511966,-52.5381931806012)
--(axis cs:1.0471975511966,-52.5381931806012)
--(axis cs:0.936966230018008,-57.7915358495645)
--(axis cs:0.826734908839419,-64.3608589455626)
--(axis cs:0.71650358766083,-63.5035322855441)
--(axis cs:0.606272266482241,-63.2976162658452)
--(axis cs:0.496040945303651,-58.5852931780614)
--(axis cs:0.385809624125062,-54.3166759039099)
--(axis cs:0.275578302946473,-47.8617916401253)
--(axis cs:0.165346981767884,-35.411344480246)
--(axis cs:0.0551156605892946,-25.5409135446061)
--(axis cs:-0.0551156605892946,-14.79816548195)
--(axis cs:-0.165346981767884,-5.49627869415472)
--(axis cs:-0.275578302946473,-2.0553544886598)
--(axis cs:-0.385809624125062,-2.47145051769509)
--(axis cs:-0.496040945303652,-7.70968375660863)
--(axis cs:-0.606272266482241,-14.371033331744)
--(axis cs:-0.71650358766083,-20.7570936216804)
--(axis cs:-0.826734908839419,-23.3846301316924)
--(axis cs:-0.936966230018008,-23.2353633399669)
--(axis cs:-1.0471975511966,-22.7519982348471)
--cycle;

\path [draw=color0, fill=color0, opacity=0.1]
(axis cs:-1.0471975511966,-19.063255589715)
--(axis cs:-1.0471975511966,-29.4810120873568)
--(axis cs:-0.936966230018008,-34.2715193897583)
--(axis cs:-0.826734908839419,-37.7711584851522)
--(axis cs:-0.71650358766083,-34.8210156949038)
--(axis cs:-0.606272266482241,-26.5178722593201)
--(axis cs:-0.496040945303652,-18.9229441105969)
--(axis cs:-0.385809624125062,-11.4768806793955)
--(axis cs:-0.275578302946473,-9.84911701970025)
--(axis cs:-0.165346981767884,-15.8721455701697)
--(axis cs:-0.0551156605892946,-25.5321399032291)
--(axis cs:0.0551156605892946,-38.8979239554533)
--(axis cs:0.165346981767884,-56.1127934800804)
--(axis cs:0.275578302946473,-67.1703271324974)
--(axis cs:0.385809624125062,-81.1308518316762)
--(axis cs:0.496040945303651,-88.8688055263556)
--(axis cs:0.606272266482241,-91.9235875612353)
--(axis cs:0.71650358766083,-91.6443497777964)
--(axis cs:0.826734908839419,-96.4565636376583)
--(axis cs:0.936966230018008,-88.4784518385123)
--(axis cs:1.0471975511966,-71.8682027011649)
--(axis cs:1.0471975511966,-50.3057249058303)
--(axis cs:1.0471975511966,-50.3057249058303)
--(axis cs:0.936966230018008,-61.3452057197951)
--(axis cs:0.826734908839419,-60.7707389252343)
--(axis cs:0.71650358766083,-60.5980779538837)
--(axis cs:0.606272266482241,-61.3552331887514)
--(axis cs:0.496040945303651,-62.2925284415788)
--(axis cs:0.385809624125062,-59.1636242096334)
--(axis cs:0.275578302946473,-50.2928810277961)
--(axis cs:0.165346981767884,-41.679831340888)
--(axis cs:0.0551156605892946,-30.4518127616432)
--(axis cs:-0.0551156605892946,-21.1979834860429)
--(axis cs:-0.165346981767884,-13.2926172147716)
--(axis cs:-0.275578302946473,-8.20984050177886)
--(axis cs:-0.385809624125062,-8.98250064423069)
--(axis cs:-0.496040945303652,-14.0729806285338)
--(axis cs:-0.606272266482241,-20.6970250995847)
--(axis cs:-0.71650358766083,-25.5191234210262)
--(axis cs:-0.826734908839419,-24.6594554729815)
--(axis cs:-0.936966230018008,-24.9550755552989)
--(axis cs:-1.0471975511966,-19.063255589715)
--cycle;

\path [draw=red!49.8039215686275!black, fill=red!49.8039215686275!black, opacity=0.1]
(axis cs:-1.0471975511966,-13.4775621313768)
--(axis cs:-1.0471975511966,-32.428190991817)
--(axis cs:-0.936966230018008,-34.5292594279107)
--(axis cs:-0.826734908839419,-35.9844438041085)
--(axis cs:-0.71650358766083,-32.4750537870735)
--(axis cs:-0.606272266482241,-28.9474915065193)
--(axis cs:-0.496040945303652,-26.0248309227754)
--(axis cs:-0.385809624125062,-29.9318453754403)
--(axis cs:-0.275578302946473,-32.7502097212677)
--(axis cs:-0.165346981767884,-42.2886140865705)
--(axis cs:-0.0551156605892946,-52.8904549664494)
--(axis cs:0.0551156605892946,-67.0111855798771)
--(axis cs:0.165346981767884,-76.0755716144616)
--(axis cs:0.275578302946473,-80.3563956157798)
--(axis cs:0.385809624125062,-92.4323279482623)
--(axis cs:0.496040945303651,-98.6907261107124)
--(axis cs:0.606272266482241,-95.0403154821288)
--(axis cs:0.71650358766083,-94.7240928758257)
--(axis cs:0.826734908839419,-87.2377404251417)
--(axis cs:0.936966230018008,-85.3060537460388)
--(axis cs:1.0471975511966,-72.8550996257074)
--(axis cs:1.0471975511966,-53.7221405799838)
--(axis cs:1.0471975511966,-53.7221405799838)
--(axis cs:0.936966230018008,-58.5519301217736)
--(axis cs:0.826734908839419,-65.7219533529484)
--(axis cs:0.71650358766083,-63.9692590663922)
--(axis cs:0.606272266482241,-61.3996936030435)
--(axis cs:0.496040945303651,-63.9320767732879)
--(axis cs:0.385809624125062,-52.1653255910741)
--(axis cs:0.275578302946473,-42.710177160733)
--(axis cs:0.165346981767884,-34.4210463190196)
--(axis cs:0.0551156605892946,-28.8966980859574)
--(axis cs:-0.0551156605892946,-15.7020930637253)
--(axis cs:-0.165346981767884,-10.3833733003655)
--(axis cs:-0.275578302946473,-6.31300646622772)
--(axis cs:-0.385809624125062,-4.34140111015916)
--(axis cs:-0.496040945303652,-4.18333805151197)
--(axis cs:-0.606272266482241,-5.91973184249647)
--(axis cs:-0.71650358766083,-5.12758298171686)
--(axis cs:-0.826734908839419,-10.1289807395589)
--(axis cs:-0.936966230018008,-11.6155143081388)
--(axis cs:-1.0471975511966,-13.4775621313768)
--cycle;

\addplot [ultra thick, black, dashed]
table {%
-1.0471975511966 -27.766653422415
-0.936966230018008 -29.6196540532391
-0.826734908839419 -29.7046702729404
-0.71650358766083 -27.3630491933635
-0.606272266482241 -22.5599806868502
-0.496040945303652 -16.3267585369783
-0.385809624125062 -8.89134405934497
-0.275578302946473 -7.95733429032118
-0.165346981767884 -14.3495584437453
-0.0551156605892946 -24.5483374824025
0.0551156605892946 -35.2940177947902
0.165346981767884 -45.0117805743886
0.275578302946473 -56.2841491640561
0.385809624125062 -62.8544846011332
0.496040945303651 -67.522243795217
0.606272266482241 -71.8467524331183
0.71650358766083 -71.8388265790354
0.826734908839419 -70.0513044853737
0.936966230018008 -64.814352038424
1.0471975511966 -58.2356673908128
};
\addlegendentry{True Value}
\addplot [ultra thick, color0, mark=*, mark size=2.0, mark options={solid,fill=color3}]
table {%
-1.0471975511966 -24.2721338385359
-0.936966230018008 -29.6132974725286
-0.826734908839419 -31.2153069790669
-0.71650358766083 -30.170069557965
-0.606272266482241 -23.6074486794524
-0.496040945303652 -16.4979623695653
-0.385809624125062 -10.2296906618131
-0.275578302946473 -9.02947876073955
-0.165346981767884 -14.5823813924707
-0.0551156605892946 -23.365061694636
0.0551156605892946 -34.6748683585483
0.165346981767884 -48.8963124104842
0.275578302946473 -58.7316040801467
0.385809624125062 -70.1472380206548
0.496040945303651 -75.5806669839672
0.606272266482241 -76.6394103749933
0.71650358766083 -76.12121386584
0.826734908839419 -78.6136512814463
0.936966230018008 -74.9118287791537
1.0471975511966 -61.0869638034976
};
\addlegendentry{OEE (ours)}
\addplot [ultra thick, red!49.8039215686275!black]
table {%
-1.0471975511966 -22.9528765615969
-0.936966230018008 -23.0723868680248
-0.826734908839419 -23.0567122718337
-0.71650358766083 -18.8013183843952
-0.606272266482241 -17.4336116745079
-0.496040945303652 -15.1040844871437
-0.385809624125062 -17.1366232427997
-0.275578302946473 -19.5316080937477
-0.165346981767884 -26.335993693468
-0.0551156605892946 -34.2962740150873
0.0551156605892946 -47.9539418329172
0.165346981767884 -55.2483089667406
0.275578302946473 -61.5332863882564
0.385809624125062 -72.2988267696682
0.496040945303651 -81.3114014420002
0.606272266482241 -78.2200045425862
0.71650358766083 -79.3466759711089
0.826734908839419 -76.4798468890451
0.936966230018008 -71.9289919339062
1.0471975511966 -63.2886201028456
};
\addlegendentry{Simulated}
\end{axis}

\end{tikzpicture}


==> DartEnv/dart_evaluation_4142.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0,0.266666666666667,0.105882352941176}
\definecolor{color3}{rgb}{0.2549, 0.6823, 0.4627}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Theta},
xmajorgrids,
xmin=-1.15191730631626, xmax=1.15191730631626,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Average returns},
ymajorgrids,
ymin=-106.406286455585, ymax=2.10066449747733,
ytick style={color=black}
]
\path [draw=black, fill=black, opacity=0.1]
(axis cs:-1.0471975511966,-18.8559551509907)
--(axis cs:-1.0471975511966,-27.8695875941962)
--(axis cs:-0.936966230018008,-30.4052226778153)
--(axis cs:-0.826734908839419,-29.908897521895)
--(axis cs:-0.71650358766083,-26.720263566886)
--(axis cs:-0.606272266482241,-23.0439019167632)
--(axis cs:-0.496040945303652,-16.8230370645434)
--(axis cs:-0.385809624125062,-13.7580030251357)
--(axis cs:-0.275578302946473,-20.239052798178)
--(axis cs:-0.165346981767884,-32.401671379012)
--(axis cs:-0.0551156605892946,-43.0570171606262)
--(axis cs:0.0551156605892946,-55.1341876030111)
--(axis cs:0.165346981767884,-68.1283325284223)
--(axis cs:0.275578302946473,-72.4090525734823)
--(axis cs:0.385809624125062,-81.6989393326927)
--(axis cs:0.496040945303651,-85.0397668084986)
--(axis cs:0.606272266482241,-88.935283200636)
--(axis cs:0.71650358766083,-86.7222143231953)
--(axis cs:0.826734908839419,-83.1466178215183)
--(axis cs:0.936966230018008,-77.9366472276308)
--(axis cs:1.0471975511966,-67.3123328082259)
--(axis cs:1.0471975511966,-58.2336955210237)
--(axis cs:1.0471975511966,-58.2336955210237)
--(axis cs:0.936966230018008,-65.0669321292164)
--(axis cs:0.826734908839419,-69.7483231401934)
--(axis cs:0.71650358766083,-71.9687234541295)
--(axis cs:0.606272266482241,-70.8418131502477)
--(axis cs:0.496040945303651,-67.2670788395692)
--(axis cs:0.385809624125062,-62.0864528497476)
--(axis cs:0.275578302946473,-53.1263944082203)
--(axis cs:0.165346981767884,-45.4802828114706)
--(axis cs:0.0551156605892946,-35.3603847740884)
--(axis cs:-0.0551156605892946,-23.9694387841712)
--(axis cs:-0.165346981767884,-13.2211214065935)
--(axis cs:-0.275578302946473,-3.97605410809775)
--(axis cs:-0.385809624125062,-2.8314696367528)
--(axis cs:-0.496040945303652,-3.07288074607547)
--(axis cs:-0.606272266482241,-7.03869442551705)
--(axis cs:-0.71650358766083,-12.5077508114754)
--(axis cs:-0.826734908839419,-17.4329893105515)
--(axis cs:-0.936966230018008,-18.1108241308253)
--(axis cs:-1.0471975511966,-18.8559551509907)
--cycle;

\path [draw=color0, fill=color0, opacity=0.1]
(axis cs:-1.0471975511966,-17.8368771440615)
--(axis cs:-1.0471975511966,-28.1392061246536)
--(axis cs:-0.936966230018008,-30.3104754374086)
--(axis cs:-0.826734908839419,-27.0200378965452)
--(axis cs:-0.71650358766083,-24.0736565705352)
--(axis cs:-0.606272266482241,-17.8339850122684)
--(axis cs:-0.496040945303652,-11.1300337210902)
--(axis cs:-0.385809624125062,-9.41042941603587)
--(axis cs:-0.275578302946473,-14.8660378333385)
--(axis cs:-0.165346981767884,-23.3339633596903)
--(axis cs:-0.0551156605892946,-33.9409742112935)
--(axis cs:0.0551156605892946,-47.0392352007273)
--(axis cs:0.165346981767884,-63.5807862835734)
--(axis cs:0.275578302946473,-78.4581631078625)
--(axis cs:0.385809624125062,-97.1864358998734)
--(axis cs:0.496040945303651,-99.9509105388278)
--(axis cs:0.606272266482241,-101.474152321355)
--(axis cs:0.71650358766083,-99.479882692786)
--(axis cs:0.826734908839419,-93.3731159117204)
--(axis cs:0.936966230018008,-77.7833710428702)
--(axis cs:1.0471975511966,-47.3838394978988)
--(axis cs:1.0471975511966,-34.281777463232)
--(axis cs:1.0471975511966,-34.281777463232)
--(axis cs:0.936966230018008,-55.0959908834641)
--(axis cs:0.826734908839419,-66.623681571042)
--(axis cs:0.71650358766083,-71.6624106101607)
--(axis cs:0.606272266482241,-71.9776210150423)
--(axis cs:0.496040945303651,-67.5814712941269)
--(axis cs:0.385809624125062,-66.3561886319973)
--(axis cs:0.275578302946473,-54.4160276232391)
--(axis cs:0.165346981767884,-45.838226397613)
--(axis cs:0.0551156605892946,-38.1880095658302)
--(axis cs:-0.0551156605892946,-28.2467440981311)
--(axis cs:-0.165346981767884,-19.6132920917879)
--(axis cs:-0.275578302946473,-11.6661425509925)
--(axis cs:-0.385809624125062,-7.61860638732108)
--(axis cs:-0.496040945303652,-7.66107121444548)
--(axis cs:-0.606272266482241,-12.3737877316573)
--(axis cs:-0.71650358766083,-16.7533429686776)
--(axis cs:-0.826734908839419,-18.0503633894292)
--(axis cs:-0.936966230018008,-17.8616542415002)
--(axis cs:-1.0471975511966,-17.8368771440615)
--cycle;

\path [draw=red!49.8039215686275!black, fill=red!49.8039215686275!black, opacity=0.1]
(axis cs:-1.0471975511966,-12.8167273921821)
--(axis cs:-1.0471975511966,-33.6349972169892)
--(axis cs:-0.936966230018008,-37.3587707235592)
--(axis cs:-0.826734908839419,-37.918563471314)
--(axis cs:-0.71650358766083,-35.3193358449701)
--(axis cs:-0.606272266482241,-24.9936707089606)
--(axis cs:-0.496040945303652,-23.7586302089764)
--(axis cs:-0.385809624125062,-26.6312728963261)
--(axis cs:-0.275578302946473,-30.9293269029626)
--(axis cs:-0.165346981767884,-44.991329070721)
--(axis cs:-0.0551156605892946,-56.342658629758)
--(axis cs:0.0551156605892946,-66.2588923942456)
--(axis cs:0.165346981767884,-73.4451013593095)
--(axis cs:0.275578302946473,-84.6525215196275)
--(axis cs:0.385809624125062,-92.7457914926398)
--(axis cs:0.496040945303651,-94.2297508821346)
--(axis cs:0.606272266482241,-97.106978109375)
--(axis cs:0.71650358766083,-95.8346188945244)
--(axis cs:0.826734908839419,-89.3025782804569)
--(axis cs:0.936966230018008,-83.9674385775424)
--(axis cs:1.0471975511966,-73.3033962869418)
--(axis cs:1.0471975511966,-54.079989306198)
--(axis cs:1.0471975511966,-54.079989306198)
--(axis cs:0.936966230018008,-61.5281960152806)
--(axis cs:0.826734908839419,-62.0847348319098)
--(axis cs:0.71650358766083,-62.9982256485735)
--(axis cs:0.606272266482241,-60.1480426862307)
--(axis cs:0.496040945303651,-56.0105236053352)
--(axis cs:0.385809624125062,-53.9447031138134)
--(axis cs:0.275578302946473,-44.9605365117058)
--(axis cs:0.165346981767884,-34.1988886538441)
--(axis cs:0.0551156605892946,-21.8054950974376)
--(axis cs:-0.0551156605892946,-17.3897991489577)
--(axis cs:-0.165346981767884,-9.61878426360884)
--(axis cs:-0.275578302946473,-3.50786942738887)
--(axis cs:-0.385809624125062,-3.8273885382562)
--(axis cs:-0.496040945303652,-3.89717321217138)
--(axis cs:-0.606272266482241,-3.060481287272)
--(axis cs:-0.71650358766083,-9.34341796169694)
--(axis cs:-0.826734908839419,-9.75419807009947)
--(axis cs:-0.936966230018008,-13.0036535496564)
--(axis cs:-1.0471975511966,-12.8167273921821)
--cycle;

\addplot [ultra thick, black, dashed]
table {%
-1.0471975511966 -23.3627713725934
-0.936966230018008 -24.2580234043203
-0.826734908839419 -23.6709434162233
-0.71650358766083 -19.6140071891807
-0.606272266482241 -15.0412981711401
-0.496040945303652 -9.94795890530942
-0.385809624125062 -8.29473633094426
-0.275578302946473 -12.1075534531379
-0.165346981767884 -22.8113963928027
-0.0551156605892946 -33.5132279723987
0.0551156605892946 -45.2472861885497
0.165346981767884 -56.8043076699464
0.275578302946473 -62.7677234908513
0.385809624125062 -71.8926960912201
0.496040945303651 -76.1534228240339
0.606272266482241 -79.8885481754419
0.71650358766083 -79.3454688886624
0.826734908839419 -76.4474704808559
0.936966230018008 -71.5017896784236
1.0471975511966 -62.7730141646248
};
\addlegendentry{True Value}
\addplot [ultra thick, color0, mark=*, mark size=2.0, mark options={solid,fill=color3}]
table {%
-1.0471975511966 -22.9880416343576
-0.936966230018008 -24.0860648394544
-0.826734908839419 -22.5352006429872
-0.71650358766083 -20.4134997696064
-0.606272266482241 -15.1038863719629
-0.496040945303652 -9.39555246776785
-0.385809624125062 -8.51451790167847
-0.275578302946473 -13.2660901921655
-0.165346981767884 -21.4736277257391
-0.0551156605892946 -31.0938591547123
0.0551156605892946 -42.6136223832787
0.165346981767884 -54.7095063405932
0.275578302946473 -66.4370953655508
0.385809624125062 -81.7713122659354
0.496040945303651 -83.7661909164773
0.606272266482241 -86.7258866681988
0.71650358766083 -85.5711466514734
0.826734908839419 -79.9983987413812
0.936966230018008 -66.4396809631671
1.0471975511966 -40.8328084805654
};
\addlegendentry{OEE (ours)}
\addplot [ultra thick, red!49.8039215686275!black]
table {%
-1.0471975511966 -23.2258623045856
-0.936966230018008 -25.1812121366078
-0.826734908839419 -23.8363807707067
-0.71650358766083 -22.3313769033335
-0.606272266482241 -14.0270759981163
-0.496040945303652 -13.8279017105739
-0.385809624125062 -15.2293307172912
-0.275578302946473 -17.2185981651757
-0.165346981767884 -27.3050566671649
-0.0551156605892946 -36.8662288893579
0.0551156605892946 -44.0321937458416
0.165346981767884 -53.8219950065768
0.275578302946473 -64.8065290156667
0.385809624125062 -73.3452473032266
0.496040945303651 -75.1201372437349
0.606272266482241 -78.6275103978029
0.71650358766083 -79.416422271549
0.826734908839419 -75.6936565561834
0.936966230018008 -72.7478172964115
1.0471975511966 -63.6916927965699
};
\addlegendentry{Simulated}
\end{axis}

\end{tikzpicture}


==> DartEnv/dartschematic.tex <==


\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-2.5,xscale=2.1]
%uncomment if require: \path (0,220); %set diagram left start at 0, and has height of 220

%Straight Lines [id:da5598931131802194] 
\draw[ultra thick]    (288,110) -- (391,110) ;
%Straight Lines [id:da11156130040470225] 
\draw[ultra thick]    (289,210) -- (390,210) ;
%Straight Lines [id:da9641974169779695] 
\draw [ultra thick, color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (339.5,110) -- (339.5,210) ;
%Straight Lines [id:da3015993328945221] 
\draw [ultra thick, color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (296,166) -- (316,166) ;
\draw [shift={(318,166)}, rotate = 180] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da12843122113925243] 
\draw[ultra thick]    (338.5,209) -- (316.94,203.49) ;
\draw [shift={(315,203)}, rotate = 374.32] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da18571667856743668] 
\draw [ultra thick, color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (296,181) -- (316,181) ;
\draw [shift={(318,181)}, rotate = 180] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9076090886574564] 
\draw [ultra thick, color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ]   (297,151) -- (317,151) ;
\draw [shift={(319,151)}, rotate = 180] [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da5947601459181651] 
\draw    (333,206) .. controls (330,197) and (341,201) .. (339,202) ;

% Text Node
\draw (297,136) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textcolor[rgb]{0.29,0.56,0.89}{$\mathbf{W}$}};
% Text Node
\draw (327,194) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\theta$};


\end{tikzpicture}


==> Kinova/kinova_robot.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}
\node [anchor=north] (image) at (0,1) {
        \includegraphics[keepaspectratio=True,width=6.2cm]{Kinova/kinovarobot.png}
    };
\end{tikzpicture}

==> Kinova/kinova_sim2real.tex <==
% This file was created by tikzplotlib v0.9.3.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0,0.266666666666667,0.105882352941176}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black, at={(1.0,1.0)}},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Goal Index},
xmin=-0.175, xmax=3.675,
xtick style={color=black},
xtick={0.5,1.5,2.5,3.5},
xticklabels={1, 2, 3, 4},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ylabel={Average Returns},
ymajorgrids,
ymin=-1.7, ymax=0.0745954702274459,
ytick style={color=black},
ytick={-1.6,-1.4,-1.2,-1,-0.8,-0.6,-0.4,-0.2,0,0.2},
yticklabels={−1.6,−1.4,−1.2,−1.0,−0.8,−0.6,−0.4,−0.2,0.0,0.2}
]
\path [draw=black, draw opacity=0.2, line width=2pt]
(axis cs:0,-0.597672)
--(axis cs:0,0);

\path [draw=black, draw opacity=0.2, line width=2pt]
(axis cs:1,-1.2834)
--(axis cs:1,0);

\path [draw=black, draw opacity=0.2, line width=2pt]
(axis cs:2,-0.9624)
--(axis cs:2,0);

\path [draw=black, draw opacity=0.2, line width=2pt]
(axis cs:3,-0.80264)
--(axis cs:3,0);

\path [draw=color0, draw opacity=0.2, line width=2pt]
(axis cs:0.25,-0.819560774920544)
--(axis cs:0.25,0);

\path [draw=color0, draw opacity=0.2, line width=2pt]
(axis cs:1.25,-1.40432473999285)
--(axis cs:1.25,0);

\path [draw=color0, draw opacity=0.2, line width=2pt]
(axis cs:2.25,-1.09458121402426)
--(axis cs:2.25,0);

\path [draw=color0, draw opacity=0.2, line width=2pt]
(axis cs:3.25,-1.06494495486414)
--(axis cs:3.25,0);

\path [draw=red!49.8039215686275!black, draw opacity=0.2, line width=2pt]
(axis cs:0.5,-0.926234433076563)
--(axis cs:0.5,0);

\path [draw=red!49.8039215686275!black, draw opacity=0.2, line width=2pt]
(axis cs:1.5,-1.49190940454892)
--(axis cs:1.5,0);

\path [draw=red!49.8039215686275!black, draw opacity=0.2, line width=2pt]
(axis cs:2.5,-1.1027486582395)
--(axis cs:2.5,0);

\path [draw=red!49.8039215686275!black, draw opacity=0.2, line width=2pt]
(axis cs:3.5,-1.20969405098886)
--(axis cs:3.5,0);

\addplot [semithick, black, opacity=0.8, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
0 -0.597672
1 -1.2834
2 -0.9624
3 -0.80264
};
\addlegendentry{True}
\addplot [semithick, color0, opacity=0.8, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
0.25 -0.819560774920544
1.25 -1.40432473999285
2.25 -1.09458121402426
3.25 -1.06494495486414
};
\addlegendentry{OEE (Ours)}
\addplot [semithick, red!49.8039215686275!black, opacity=0.8, mark=*, mark size=2.5, mark options={solid}, only marks]
table {%
0.5 -0.926234433076563
1.5 -1.49190940454892
2.5 -1.1027486582395
3.5 -1.20969405098886
};
\addlegendentry{Simulated}
\end{axis}

\end{tikzpicture}

